ReLU-QP: A GPU-Accelerated Quadratic Programming Solver for Model-Predictive Control

We present ReLU-QP, a GPU-accelerated solver for quadratic programs (QPs) that is capable of solving high-dimensional control problems at real-time rates. ReLU-QP is derived by exactly reformulating the Alternating Direction Method of Multipliers (ADMM) algorithm for solving QPs as a deep, weight-tied neural network with rectified linear unit (ReLU) activations. This reformulation enables the deployment of ReLU-QP on GPUs using standard machine-learning toolboxes. We evaluate the performance of ReLU-QP across three model-predictive control (MPC) benchmarks: stabilizing random linear dynamical systems with control limits, balancing an Atlas humanoid robot on a single foot, and tracking whole-body reference trajectories on a quadruped equipped with a six-degree-of-freedom arm. These benchmarks indicate that ReLU-QP is competitive with state-of-the-art CPU-based solvers for small-to-medium-scale problems and offers order-of-magnitude speed improvements for larger-scale problems.

==> figures/random_mixed_qp_init_low_tol.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{chocolate2267451}{RGB}{226,74,51}
\definecolor{dimgray85}{RGB}{85,85,85}
\definecolor{gainsboro229}{RGB}{229,229,229}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{mediumpurple152142213}{RGB}{152,142,213}
\definecolor{steelblue52138189}{RGB}{52,138,189}

\begin{axis}[
axis background/.style={fill=gainsboro229},
axis line style={white},
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0.03,0.97)},
  anchor=north west,
  draw=lightgray204,
  fill=gainsboro229
},
log basis x={10},
log basis y={10},
tick align=outside,
tick pos=left,
x grid style={white},
xlabel={Problem Size},
xmajorgrids,
xmin=7, xmax=3000,
xmode=log,
xtick style={color=dimgray85},
xtick = {1e1, 1e2, 1e3},
y grid style={white},
ylabel={Solve Time (s)},
ymajorgrids,
ymin=5e-06, ymax=50,
ymode=log,
ytick style={color=dimgray85},
ytick={1e-5, 1e-4, 1e-3, 1e-2, 1e-1, 1e0, 1e1}
]
\path [draw=chocolate2267451, semithick]
(axis cs:10,3.16373870400655e-05)
--(axis cs:10,4.49176129599345e-05);

\path [draw=chocolate2267451, semithick]
(axis cs:18,6.67645743547738e-05)
--(axis cs:18,7.98774256452261e-05);

\path [draw=chocolate2267451, semithick]
(axis cs:32,0.000159121074773577)
--(axis cs:32,0.000209752125226423);

\path [draw=chocolate2267451, semithick]
(axis cs:58,0.000544782589340305)
--(axis cs:58,0.000867707877326362);

\path [draw=chocolate2267451, semithick]
(axis cs:105,0.00222384524635756)
--(axis cs:105,0.0030704254203091);

\path [draw=chocolate2267451, semithick]
(axis cs:190,0.00732084414074199)
--(axis cs:190,0.00812233519259134);

\path [draw=chocolate2267451, semithick]
(axis cs:342,0.0278731535403038)
--(axis cs:342,0.0289218204596962);

\path [draw=chocolate2267451, semithick]
(axis cs:616,0.126856289767828)
--(axis cs:616,0.130272819298839);

\path [draw=chocolate2267451, semithick]
(axis cs:1110,0.665816792417729)
--(axis cs:1110,0.742027026382271);

\path [draw=chocolate2267451, semithick]
(axis cs:2000,4.67778772661565)
--(axis cs:2000,4.85767741311768);

\path [draw=steelblue52138189, semithick]
(axis cs:10,1.43475431096791e-05)
--(axis cs:10,3.12484568903209e-05);

\path [draw=steelblue52138189, semithick]
(axis cs:18,2.82041803386324e-05)
--(axis cs:18,4.12800863280343e-05);

\path [draw=steelblue52138189, semithick]
(axis cs:32,5.18204089992706e-05)
--(axis cs:32,6.97969910007294e-05);

\path [draw=steelblue52138189, semithick]
(axis cs:58,0.000149175083785807)
--(axis cs:58,0.00023967278288086);

\path [draw=steelblue52138189, semithick]
(axis cs:105,0.000518054700281193)
--(axis cs:105,0.00072163423305214);

\path [draw=steelblue52138189, semithick]
(axis cs:190,0.00119981388637187)
--(axis cs:190,0.00144826271362813);

\path [draw=steelblue52138189, semithick]
(axis cs:342,0.00454190207635111)
--(axis cs:342,0.00485487859031555);

\path [draw=steelblue52138189, semithick]
(axis cs:616,0.01672682028842)
--(axis cs:616,0.0177936452449133);

\path [draw=steelblue52138189, semithick]
(axis cs:1110,0.0737008703546114)
--(axis cs:1110,0.0839698831787219);

\path [draw=steelblue52138189, semithick]
(axis cs:2000,0.447462397012349)
--(axis cs:2000,0.485711680120984);

\path [draw=mediumpurple152142213, semithick]
(axis cs:10,0.000890624961723037)
--(axis cs:10,0.00242009717421567);

\path [draw=mediumpurple152142213, semithick]
(axis cs:18,0.00113300090141934)
--(axis cs:18,0.00250765831024978);

\path [draw=mediumpurple152142213, semithick]
(axis cs:32,0.00139226232246331)
--(axis cs:32,0.00284437346060304);

\path [draw=mediumpurple152142213, semithick]
(axis cs:58,0.000993966508163534)
--(axis cs:58,0.00277479077630016);

\path [draw=mediumpurple152142213, semithick]
(axis cs:105,0.00111311882814403)
--(axis cs:105,0.00237051637840757);

\path [draw=mediumpurple152142213, semithick]
(axis cs:190,0.000601961706609744)
--(axis cs:190,0.00118499294389042);

\path [draw=mediumpurple152142213, semithick]
(axis cs:342,0.000696418127420173)
--(axis cs:342,0.000816919468744223);

\path [draw=mediumpurple152142213, semithick]
(axis cs:616,0.00161250858574366)
--(axis cs:616,0.0025891255105485);

\path [draw=mediumpurple152142213, semithick]
(axis cs:1110,0.00475810123127633)
--(axis cs:1110,0.00503902078775631);

\path [draw=mediumpurple152142213, semithick]
(axis cs:2000,0.0106786299743599)
--(axis cs:2000,0.0110680259517485);

\addplot [semithick, chocolate2267451, dashed, mark=*, mark size=3, mark options={solid}]
table {%
10 3.82775e-05
18 7.3321e-05
32 0.0001844366
58 0.000706245233333333
105 0.00264713533333333
190 0.00772158966666667
342 0.028397487
616 0.128564554533333
1110 0.7039219094
2000 4.76773256986667
};
\addlegendentry{OSQP}
\addplot [semithick, steelblue52138189, dashed, mark=*, mark size=3, mark options={solid}]
table {%
10 2.2798e-05
18 3.47421333333333e-05
32 6.08087e-05
58 0.000194423933333333
105 0.000619844466666667
190 0.0013240383
342 0.00469839033333333
616 0.0172602327666667
1110 0.0788353767666667
2000 0.466587038566667
};
\addlegendentry{ProxQP}
\addplot [semithick, mediumpurple152142213, dashed, mark=*, mark size=3, mark options={solid}]
table {%
10 0.00165536106796935
18 0.00182032960583456
32 0.00211831789153318
58 0.00188437864223185
105 0.0017418176032758
190 0.000893477325250084
342 0.000756668798082198
616 0.00210081704814608
1110 0.00489856100951632
2000 0.0108733279630542
};
\addlegendentry{ReLU-QP}
\end{axis}

\end{tikzpicture}

